Networked Digital Public Goods Games with Heterogeneous Players and Convex Costs

In the digital age, resources such as open-source software and publicly accessible databases form a crucial category of digital public goods, providing extensive benefits for Internet. This paper investigates networked public goods games involving heterogeneous players and convex costs, focusing on the characterization of Nash Equilibrium (NE). In these games, each player can choose her effort level, representing her contributions to public goods. Network structures are employed to model the interactions among participants. Each player's utility consists of a concave value component, influenced by the collective efforts of all players, and a convex cost component, determined solely by the individual's own effort. To the best of our knowledge, this study is the first to explore the networked public goods game with convex costs. Our research begins by examining welfare solutions aimed at maximizing social welfare and ensuring the convergence of pseudo-gradient ascent dynamics. We establish the presence of NE in this model and provide an in-depth analysis of the conditions under which NE is unique. We also delve into comparative statics, an essential tool in economics, to evaluate how slight modifications in the model--interpreted as monetary redistribution--affect player utilities. In addition, we analyze a particular scenario with a predefined game structure, illustrating the practical relevance of our theoretical insights. Overall, our research enhances the broader understanding of strategic interactions and structural dynamics in networked public goods games, with significant implications for policy design in internet economic and social networks.

==> Contents/Proofs/lem_argmax_Lipschitz.tex <==
\begin{proof}
\label{prf:lem:argmax:Lipschitz}
The existence and uniqueness of the maximum solution are readily established, as it is a well-known property that a strongly concave function always possesses a unique maximum within a bounded, closed, and convex set. 

The proof of property of Lipschitzness will be presented in the subsequent discussion.

Let $x_i = x(c_i)$ for $i=1,2$ and denote $y = \frac{x_1 + x_2}{2}$. We know $y\in X$ by convexity of $X$. By the optimality of $x_i$ we have,
\begin{align}
    g(c_1,x_1) + f(x_1) \ge& g(c_1,y) + f(y);\label{lemma4.6-ineq1}
    \\
    g(c_2,x_2) + f(x_2) \ge& g(c_2,y) + f(y).\label{lemma4.6-ineq2}
\end{align}
Combining (\ref{lemma4.6-ineq1}) and (\ref{lemma4.6-ineq2}), we know that
\begin{align}
    g(c_1,x_1) + g(c_2,x_2) - \left[ g(c_1,y) + g(c_2,y)\right] \ge& 2f(\frac{x_1+x_2}{2}) - (f(x_1) + f(x_2)) \ge \frac{\alpha}{4}||x_1 - x_2||^2,\label{lemma4.6-ineq3}
\end{align}
where the last inequality is satisfied by the $\alpha$-concavity of $f(x)$.

By concavity of $g(c,x)$ on $x$, we also have
\begin{align}
    &g(c_1,x_1) + g(c_2,x_2) - \left[ g(c_1,y) + g(c_2,y)\right] \nonumber\\
    \le& g(c_1,x_1) + g(c_2,x_2) - \frac{1}{2}\left[ g(c_1,x_1) + g(c_2,x_2) + g(c_1,x_2) + g(c_2,x_1) \right]
    \nonumber\\
    =& \frac{1}{2}(g(c_1,x_1) + g(c_2,x_2) - g(c_1,x_2) - g(c_2,x_1))
    \nonumber\\
    =& \frac{1}{2} \int_{L_c} \int_{L_x} \ \bm{r}_c^T \frac{\partial g}{\partial c \partial x}(c,x) \bm{r}_x \ dc dx
    \nonumber\\
    \le& \frac{L}{2} ||c_1 - c_2||\cdot ||x_1 - x_2||\label{lemma4.6-ineq4}
\end{align}
where $L_c, L_x$ represent the straight line between $c_1,c_2$ and $x_1,x_2$, respectively, and $\bm{r}_c$ and $\bm{r}_x$  denote the unit vector with direction $c_2 - c_1$ and $x_2 - x_1$.
Combining (\ref{lemma4.6-ineq3}) and (\ref{lemma4.6-ineq4}), we derive that
\begin{align*}
    ||x_1 - x_2|| \le \frac{2L}{\alpha} ||c_1 - c_2||,
\end{align*}
which completes the proof for $\frac{2L}{\alpha}$-Lipschitzness of $x(c)$.
\end{proof}

==> Contents/Theorems/lem_argmax_Lipschitz.tex <==
\begin{restatable}{lemma}{lemArgmaxLipschitz}
\label{lem:argmax:Lipschitz}
Let function $u(c,x) = g(c,x) + f(x)$ be defined on a bounded, closed, and convex set $X$. Suppose that $g(c,x)$ is concave on $x$, twice differentiable almost everywhere with 
$$\sigma_{max}( \frac{\partial g}{\partial c\partial x} ) \coloneqq \sup_{||r_c|| = ||r_x|| = 1} r_c^T \frac{\partial g}{\partial c\partial x} r_x \le L$$ for some positive real number $L$ and $f(x)$ is an $\alpha$-concave function. We denote the maximum solution of $u(c, x)$ by $x(c) = \arg\max_{x\in X} u(c,x)$. Thus, $x(c)$ not only exists and is unique, but it is also $\frac{2L}{\alpha}$-Lipschitz continuous with respect to $c$.
\end{restatable}

==> Contents/_authors.tex <==

\author{Anonymous Authors}
\institute{Anonymous Institute}

% \author{First Author\inst{1}\orcidID{0000-1111-2222-3333} \and
% Second Author\inst{2,3}\orcidID{1111-2222-3333-4444} \and
% Third Author\inst{3}\orcidID{2222--3333-4444-5555}}
% %
% \authorrunning{F. Author et al.}
% % First names are abbreviated in the running head.
% % If there are more than two authors, 'et al.' is used.
% %
% \institute{Princeton University, Princeton NJ 08544, USA \and
% Springer Heidelberg, Tiergartenstr. 17, 69121 Heidelberg, Germany
% \email{lncs@springer.com}\\
% \url{http://www.springer.com/gp/computer-science/lncs} \and
% ABC Institute, Rupert-Karls-University Heidelberg, Heidelberg, Germany\\
% \email{\{abc,lncs\}@uni-heidelberg.de}}
